System of evolution equations for quark and gluon jet quenching with broadening

We propose a system of evolution equations that describe in-medium time-evolution of transverse-momentum-dependent quark and gluon fragmentation functions. Furthermore, we solve this system of equations using Monte Carlo methods. We then quantify the obtained solutions in terms of a few characteristic features, namely the average transverse momentum $\langle |k|\rangle$ and energy contained in a cone, which allow us to see different behaviour of quark and gluon initiated final-state radiation. In particular, the later allows us to conclude that in the gluon-initiated processes there is less energy in a cone, so that the quark jet is more collimated.

==> KTparams.tex <==
% Paragraph on parameters by Konrad
\paragraph{\textbf{Medium parameters:}}
We agreed on a run with fixed medium parameters. These are the following
\begin{equation}
    g_{\rm med} = 2\,, \;\;\; T = 250\, {\rm MeV }\,,\;\;\; {\rm and}\;\; L = 5\, {\rm fm} \,.     
\end{equation}
In a thermal medium (at LO) we have,
\begin{align}
    m_D^2 &= \left(1+\frac{n_f}{6}\right) g_{\rm med}^2 T^2 = \frac{3}{2} g_{\rm med}^2 T^2 \,,\\
    n_0 &= \left(1+\frac{n_f}{6}\right) T^3 = \frac{3}{2} T^3 \,,\\
    \hat{q} &= \frac{g^2_{\rm med}}{4\pi} N_c m_D^2 T \,.
\end{align}

\paragraph{\textbf{Scattering potential:}}
The scattering potential $\mathcal{C}_i({\boldsymbol l})$ ($i=q,g$), defined above is given by
\begin{equation}
    \mathcal{C}_i(\lb,t) = - C_i \sigma(\lb,t) \,,
\end{equation}
where $C_q = C_F$ for quarks and $C_g=C_A=N_c$ for gluons, and $\sigma(\lb,t)$ is related to the elastic scattering potential of the medium. In transverse coordinate space, it reads 
\begin{equation}
    \sigma(\r,t) = \int \frac{\rmd^2 \q}{(2\pi^2)} \, \frac{\rmd^2 \sigma_{\rm el}}{\rmd^2 \q} \left(1 - \rme^{i \q \cdot \r} \right) \,,
\end{equation}
where we typically employ two models for the scattering potential
\begin{align}
    \left( \frac{\rmd^2\sigma_{\rm el}}{\rmd^2 \q}\right)^\text{GW} &= \frac{g^4 n_0}{(\q^2 + \mu^2)^2} \,,\\
    \left( \frac{\rmd^2 \sigma_{\rm el}}{\rmd^2 \q}\right)^\text{HTL} &= \frac{g^2 m_D^2 T}{\q^2(\q^2 + m_D^2)} \,.
\end{align}
Hence, in transverse momentum space, we find
\begin{equation}
    \sigma(\lb,t) = \int \rmd^2 \r \, \rme^{-\lb \cdot \r} \sigma(\r,t) = - \left[\frac{\rmd^2\sigma_{\rm el}}{\rmd^2 \lb} - (2\pi)^2 \delta(\lb) \int \frac{\rmd^2 \q}{(2\pi)^2} \frac{\rmd^2\sigma_{\rm el}}{\rmd^2 \q} \right] \,.
\end{equation}

